Linear Coding for Gaussian Two-Way Channels

We consider linear coding for Gaussian two-way channels (GTWCs), in which each user generates the transmit symbols by linearly encoding both its message and the past received symbols (i.e., the feedback information) from the other user. In Gaussian one-way channels (GOWCs), Butman has proposed a well-developed model for linear encoding that encapsulates feedback information into transmit signals. However, such a model for GTWCs has not been well studied since the coupling of the encoding processes at the users in GTWCs renders the encoding design non-trivial and challenging. In this paper, we aim to fill this gap in the literature by extending the existing signal models in GOWCs to GTWCs. With our developed signal model for GTWCs, we formulate an optimization problem to jointly design the encoding/decoding schemes for both the users, aiming to minimize the weighted sum of their transmit powers under signal-to-noise ratio constraints. First, we derive an optimal form of the linear decoding schemes under any arbitrary encoding schemes employed at the users. Further, we provide new insights on the encoding design for GTWCs. In particular, we show that it is optimal that one of the users (i) does not transmit the feedback information to the other user at the last channel use, and (ii) transmits its message only over the last channel use. With these solution behaviors, we further simplify the problem and solve it via an iterative two-way optimization scheme. We numerically demonstrate that our proposed scheme for GTWCs achieves a better performance in terms of the transmit power compared to the existing counterparts, such as the non-feedback scheme and one-way optimization scheme.

==> asymmetric.tex <==
\section{Gaussian Two-way Channels}


% \textbf{Notes.} We focus on a one-way feedback scheme employing own signal removal and other message removal in asymmetric two-way channels. We want to show that this feedback scheme is superior to the two independent one-way channels and no message removal case in terms of minimizing a weight sum of powers under SNR constraints.

\subsection{Signal Transmission Model}



Suppose we have a two-way channel between two users, User 1 and User 2. 
We consider that User 1 transmits $x_1[k]$ constrained as $\mathbb{E}[\vert x_1[k] \vert^2] \leq P_1$  and User 2 transmits $x_2[k]$ constrained as $\mathbb{E}[\vert x_2[k] \vert^2] \leq P_2$  at time $k$.
The received signal at User 2 at time $k$ is given by
\begin{align}
    {y}_2[k] = x_1[n] + n_1[k],
    \label{eq:y2}
\end{align}
where ${n}_1[k]$ is additive white Gaussian noise distributed as $\mathcal{CN}(0,\sigma_1^2)$. The received signal at User 1 at time $k$ is given by
\begin{align}
    {y}_1[k] = x_2[k] + {n}_2[k],
    \label{eq:y1}
\end{align}
where ${n}_2[k]$ is additive white Gaussian noise distributed as $\mathcal{CN}(0,\sigma_2^2)$.
In vector form, these can be written as
\begin{align}
    {\bf y}_2 & = {\bf x}_1 + {\bf n}_1,
    \\
    {\bf y}_1 & = {\bf x}_2 + {\bf n}_2.
\end{align}


We assume that User 1 and 2 perform linear encoding and decoding of blocklength $N$. User $i$, for $i=1,2$, has a message $m_i \in \mathcal{M}_i$ such that $\mathbb{E}[m_i] = 0$ and $\mathbb{E}[\vert m_i \vert^2] = 1$. 
%
We consider an \textit{asymmetric} two-way channel where $P_2/\sigma_{2}^2 > P_1/\sigma_{1}^2$. We assume that User 1 employs a feedback scheme, while User 2 provides feedback information for User 1. We expect to improve the performance of User 1 by sacrificing that of User 2.

User $1$ and $2$ will construct its transmit signal, respectively, as
\begin{align}
    {\bf x}_1 & = {\bf g}_1 m_1 + {\bf F}_1 ({\bf y}_1 - {\bf F}_2 {\bf x}_1)
    \\
    & = {\bf g}_1 m_1 + {\bf F}_1 ({\bf g}_2 m_2 + {\bf F}_2 {\bf n}_1  + {\bf n}_2 ) 
    % \tilde{{\bf y}}_1 - diag({\bf F}_1 {\bf g}_2) \hat {\bf m}_2, 
    \label{eq:x1}
    \\
    {\bf x}_2 & = {\bf g}_2 m_2 + {\bf F}_2 {\bf y}_2.
    \label{eq:x2}
\end{align}
where ${\bf F}_1$ and ${\bf F}_2$ are strictly lower triangular matrices, respectively.
% We consider ${\bf F}_1 {\bf g}_2 = {\bf 0}.$
% ${\bf F}_1$ is a strictly lower triangular matrix, while ${\bf F}_2$ is a sparse matrix where only the elements on the first below diagonal are non-zero, i.e.,
% \begin{equation}
% {\bf F}_1 = \begin{bmatrix}
% 0 & 0 & 0 & ... & 0\\
% f_{1,2,1} & 0 & 0 & ... & 0 \\
% f_{1,3,1} & f_{1,3,2} & 0 & ... & 0  \\
% \vdots & \vdots & \ddots & & 0 \\
% f_{1,N,1} & f_{1,N,2} & ... & f_{1,N,N-1}
% \end{bmatrix} \in \mathbb{C}^{N \times N},
% \quad
% {\bf F}_2 = \begin{bmatrix}
% 0 & 0 & 0 & ... & 0\\
% f_{2,2} & 0 & 0 & ... & 0 \\
% 0 & f_{2,3} & 0 & ... & 0  \\
% \vdots & \vdots & \ddots & & 0 \\
% 0 & 0 & ... & f_{2,N} & 0
% \end{bmatrix} \in \mathbb{C}^{N \times N}.
% \end{equation}
% In \eqref{eq:x1}, $\tilde{{\bf y}}_1$ is an effective received signal obtained by removing ${\bf x}_1$ portion from ${\bf y}_1$. 
% Let $\tilde{{\bf y}}_1 = {\bf y}_1 - {\bf F}_2 {\bf x}_1$.
% Furthermore, User 1 estimates the message $m_2$ at each channel use and try to subtract the portion of $m_2$.
% We can rewrite the transmit signals as
% \begin{align}
%     {\bf x}_1 
%     % & = {\bf g}_1 m_1 + {\bf F}_1 \tilde{{\bf y}}_1 - diag({\bf F}_1 {\bf g}_2) \hat {\bf m}_2, 
%     % \\
%     & = {\bf g}_1 m_1 + {\bf F}_1 ({\bf g}_2 m_2 + {\bf F}_2 {\bf n}_1  + {\bf n}_2 ) 
%     % - diag({\bf F}_1 {\bf g}_2) \hat {\bf m}_2
%     % \\
%     % & = {\bf g}_1 m_1 + {\bf F}_1 ({\bf F}_2 {\bf n}_1  + {\bf n}_2 ) 
%     % + diag({\bf F}_1 {\bf g}_2)  {\bf e}_2
%     \\
%     {\bf x}_2 & = {\bf g}_2 m_2 + {\bf F}_2 {\bf y}_2.
% \end{align}
% where ${\bf e}_2 = m_2 {\bf s} - \hat {\bf m}_2$ denotes a vector collecting message estimation errors with ${\bf s} = [0,1,...,1]^T$.
%
The received signals at User 2 and User 1 are then expressed, respectively, as
\begin{align}
    {\bf y}_2 
    % & = {\bf g}_1 m_1 + {\bf F}_1 ({\bf F}_2 {\bf n}_1  + {\bf n}_2 ) + diag({\bf F}_1 {\bf g}_2)  {\bf e}_2  + {\bf n}_1,
    % \\
    % & = {\bf g}_1 m_1 + {\bf F}_1 ({\bf y}_1 - {\bf F}_2 {\bf x}_1)+ {\bf n}_1,
    % \\
    & = {\bf g}_1 m_1  + {\bf F}_1 {\bf g}_2 m_2 +
    ({\bf I} + {\bf F}_1{\bf F}_2){\bf n}_1 + {\bf F}_1{\bf n}_2 
    % + diag({\bf F}_1 {\bf g}_2)  {\bf e}_2
    \\
    {\bf y}_1 & = {\bf g}_2 m_2 + {\bf F}_2 {\bf y}_2  + {\bf n}_2
\end{align}

Using these equations, we have the power expressions for User 1 and 2 as
\begin{align}
    \mathbb{E}[\|{\bf x}_1\|^2] 
    % &= \mathbb{E}[\|{\bf g}_1 m_1 + ({\bf F}_1 - diag({\bf F}_1 {\bf g}_2) {\bf W}_2) {\bf F}_2 {\bf n}_1
    % + ({\bf F}_1 - diag({\bf F}_1 {\bf g}_2) {\bf W}_2) {\bf n}_2\|^2]
    % \nonumber
    % \\
    &= \|{\bf g}_1\|^2 +  \|{\bf F}_1 {\bf g}_2 \|^2 +  \|{\bf F}_1 {\bf F}_2 \|_F^2  \sigma_1^2
    + \| {\bf F}_1 \|_F^2  \sigma_2^2
    \\
% \end{align}
% and
% \begin{align}
    \mathbb{E} \|{\bf x}_2\|^2] 
    &=  \mathbb{E} \big[ \|{\bf g}_{2} m_2 + {\bf F}_2 \big( {\bf g}_1 m_1  + {\bf F}_1 {\bf g}_2 m_2 +
    ({\bf I} + {\bf F}_1{\bf F}_2){\bf n}_1 + {\bf F}_1{\bf n}_2  \big)  \|^2 \big]
    \nonumber
    \\
    &= \| ({\bf I} + {\bf F}_2 {\bf F}_1 ) {\bf g}_2\|^2 + \|{\bf F}_2{\bf g}_1\|^2
    + 
    \| {\bf F}_2( {\bf I} + {\bf F}_1{\bf F}_2 ) \|_F^2 \sigma_1^2
    + \| {\bf F}_2{\bf F}_1 \|_F^2 \sigma_2^2  
    % \|{\bf g}_2\|^2 + \|{\bf F}_2{\bf g}_1\|^2
    % + 
    % \| {\bf F}_2( {\bf I} + {\bf F}_1{\bf F}_2 ) \|_F^2 \sigma_1^2
    % + \| {\bf F}_2{\bf F}_1 \|_F^2 \sigma_2^2
\end{align}


\subsection{Optimal Decoding}
% User 1 estimates $m_2$ at each channel use $k$  using $\{ y_1[j]  \}_{j=1}^k$.

We assume that User 1 estimates $m_2$ such that $ {\hat m}_2 = {\bf w}_{2}^H ({\bf y}_1 - {\bf F}_2 {\bf x}_1)$.
The SNR used to estimate $m_2$ is then
\begin{align}
    {\rm SNR}_2 = \frac{\vert {\bf w}_{2}^H {\bf g}_2 \vert^2} 
    {{\bf w}_{2}^H {\bf Q}_2 {\bf w}_{2}},
\end{align}
where 
\begin{align}
    {\bf Q}_2 = {\bf F}_2 {\bf F}_2^H \sigma_1^2 + \sigma_2^2 {\bf I}.
\end{align}
% The optimal combining vector (for both maximizing and minimizing MSE of message estimation) is
% \begin{align}
%     {\bf w}_{2} = \frac{{\bf Q}_2^{-1} {\bf g}_2}
%     { {\bf g}_2^H {\bf Q}_2^{-1} {\bf g}_2}
% \end{align}
% Plugging in, we get
% \begin{align}
%       {\rm SNR}_2 =  {\bf g}_2^H {\bf Q}_2^{-1} {\bf g}_2.
% \end{align}


% We denote the $k$ partial collections of ${\bf y}_1$ as ${\bf y}_1^{(k)} = [y_1[1], ..., y_1[k]]^T \in \mathbb{C}^{k}$ given by
% \begin{align}
%     {\bf y}_1^{(k)} =  {\bf g}_2^{(k)} m_2 + {\bf F}_2^{(k)} ({\bf x}_1^{(k)} + {\bf n}_1^{(k)})  + {\bf n}_2^{(k)}
% \end{align}
% At each channel use $k$, $k=1,...,N-1$, we assume that User 1  estimates $m_2$ such that $ {\hat m}_2[k]= {\bf w}_{2,k}^H ({\bf y}_1^{(k)} - {\bf F}_2^{(k)} {\bf x}_1^{(k)})$.
% The SNR used to estimate $m_2$ at channel use $k$ is then
% \begin{align}
%     {\rm SNR}_2^{(k)} = \frac{\vert {\bf w}_{2,k}^H {\bf g}_2^{(k)} \vert^2} 
%     {{\bf w}_{2,k}^H {\bf Q}_2^{(k)} {\bf w}_{2,k}},
% \end{align}
% where 
% \begin{align}
%     {\bf Q}_2^{(k)} = {\bf F}_2^{(k)} {{\bf F}_2^{(k)}}^H \sigma_1^2 + \sigma_2^2 {\bf I}_k.
% \end{align}
% The optimal combining vector (for both maximizing and minimizing MSE of message estimation) is
% \begin{align}
%     {\bf w}_{2,k} = \frac{{{\bf Q}_2^{(k)}}^{-1} {\bf g}_2^{(k)}}
%     { {{\bf g}_2^{(k)}}^H {{\bf Q}_2^{(k)}}^{-1} {\bf g}_2^{(k)}}
% \end{align}
% Plugging in, we get
% \begin{align}
%       {\rm SNR}_2^{(k)} =  {{\bf g}_2^{(k)}}^H {{\bf Q}_2^{(k)}}^{-1} {\bf g}_2^{(k)}.
% \end{align}

% We define an aggregate combining matrix ${\bf W}_2$ with the $k+1$-th row representing the linear
% combiner at channel use $k$ (filling zeros in the rest of entries at each row) as
% \begin{equation}
%     {\bf W}_2 = \begin{bmatrix}
% 0 & 0 & 0& ...& 0\\
% {\bf w}_{2,1}^H & 0 & 0& ...& 0 \\
% \multicolumn{2}{c}{ {\bf w}_{2,2}^H} & 0& ...& 0  \\
% \vdots & \vdots  & \vdots  & ...& 0\\
% \multicolumn{4}{c}{{\bf w}_{2,N-1}^H} & 0
% \end{bmatrix}.
% \end{equation}

% Note that ${\bf w}_{2,k}^H {\bf g}_2^{(k)} = 1$. The message estimate vector is denoted by $\hat {\bf m}_2 = [0, {\hat m_2}[1], ..., {\hat m_2}[N-1]]^T$.
% The compact form is
% \begin{equation}
%     \hat {\bf m}_2 = {\bf W}_2 ({\bf y}_1 - {\bf F}_2 {\bf x}_1) 
%     = {\bf W}_2 ({\bf g}_2 m_2 + {\bf F}_2 {\bf n}_1 + {\bf n}_2)
%     =  m_2 {\bf s} + {\bf W}_2 ( {\bf F}_2 {\bf n}_1 + {\bf n}_2)
% \end{equation}
% where ${\bf s} = [0, 1, ...,1]^T$. 
% The message estimation error vector is then
% \begin{equation}
%     {\bf e}_2 = m_2 {\bf s} -  \hat {\bf m}_2 = - {\bf W}_2 ( {\bf F}_2 {\bf n}_1 + {\bf n}_2)
% \end{equation}
% Plugging in,
% we can rewrite the transmit signal of User 1 as
% \begin{align}
%     {\bf x}_1 
%     & = {\bf g}_1 m_1 + {\bf F}_1 ({\bf F}_2 {\bf n}_1  + {\bf n}_2 ) 
%     - diag({\bf F}_1 {\bf g}_2) {\bf W}_2 ( {\bf F}_2 {\bf n}_1 + {\bf n}_2)
%     \\
%     & = {\bf g}_1 m_1 + ({\bf F}_1 - diag({\bf F}_1 {\bf g}_2) {\bf W}_2) {\bf F}_2 {\bf n}_1
%     + ({\bf F}_1 - diag({\bf F}_1 {\bf g}_2) {\bf W}_2) {\bf n}_2
%  \end{align}

In the same way, we assume that User 2 estimates $m_1$ such that  $ {\hat m}_1 = {\bf w}_{1}^H ({\bf y}_2 - {\bf F}_1 {\bf g}_2 m_2)$.
% $ {\hat m}_1 = {\bf w}_{1}^H {\bf y}_2$.
% , where
% \begin{align}
%     {\bf y}_2 = {\bf g}_1 m_1 + ({\bf F}_1{\bf F}_2 - diag({\bf F}_1 {\bf g}_2) {\bf W}_2{\bf F}_2 + {\bf I})  {\bf n}_1
%     + ({\bf F}_1 - diag({\bf F}_1 {\bf g}_2) {\bf W}_2) {\bf n}_2
% \end{align}
%
The SNR used to estimate $m_1$ is then
\begin{align}
    {\rm SNR}_1 = \frac{\vert {\bf w}_{1}^H {\bf g}_1 \vert^2} 
    {{\bf w}_{1}^H {\bf Q}_1 {\bf w}_{1}},
\end{align}
where 
\begin{align}
    {\bf Q}_1 & = ({\bf I} + {\bf F}_1{\bf F}_2) ({\bf I} + {\bf F}_1{\bf F}_2)^H \sigma_1^2 
    % \\
    % & \hspace{1cm}
    + {\bf F}_1 {\bf F}_1^H \sigma_2^2.
\end{align}
% \begin{align}
%     {\bf Q}_1 & = ({\bf F}_1{\bf F}_2 - diag({\bf F}_1 {\bf g}_2) {\bf W}_2{\bf F}_2 + {\bf I}) ({\bf F}_1{\bf F}_2 - diag({\bf F}_1 {\bf g}_2) {\bf W}_2{\bf F}_2 + {\bf I})^H \sigma_1^2 
%     \\
%     & \hspace{1cm}
%     + ({\bf F}_1 - diag({\bf F}_1 {\bf g}_2) {\bf W}_2) ({\bf F}_1 - diag({\bf F}_1 {\bf g}_2) {\bf W}_2)^H \sigma_2^2.
% \end{align}
The optimal combining vector (for both maximizing and minimizing MSE of message estimation) is
\begin{align}
    {\bf w}_{i} = \frac{{\bf Q}_i^{-1} {\bf g}_i}
    { {\bf g}_i^H {{\bf Q}_i}^{-1} {\bf g}_i}, \quad i=1,2
\end{align}
Plugging in, we get
\begin{align}
      {\rm SNR}_i =  {\bf g}_i^H {\bf Q}_i^{-1} {\bf g}_i, \quad i=1,2
\end{align}





% \begin{bmatrix}
% 0 \\
% {\bf w}_{2,1}^H {\bf y}_1^{(1)}  \\
% {\bf w}_{2,2}^H {\bf y}_1^{(2)}   \\
% \vdots\\
% {\bf w}_{2,N-1}^H {\bf y}_1^{(N-1)}
% \end{bmatrix}
% = \begin{bmatrix}
% 0 \\
% m_2 + {\bf w}_{2,1}^H ({\bf F}_2^{(k)} {\bf n}_1^{(k)}  + {\bf n}_2^{(k)})
%   \\
% {\bf w}_{2,2}^H {\bf y}_1^{(2)}   \\
% \vdots\\
% {\bf w}_{2,N-1}^H {\bf y}_1^{(N-1)}
% \end{bmatrix}

% \subsection{Power Expressions}



\section{Optimization}

The overall optimization problem is
\begin{align}
    & 
    \underset{{\bf g}_1, {\bf F}_1, {\bf g}_2, {\bf F}_2}
    {\text{minimize}} & & 
 \alpha \mathbb{E}\big[\|{\bf x}_1 \|^2\big] + (1-\alpha) \mathbb{E}\big[\|{\bf x}_2 \|^2\big]
 \label{opt:obj}
\\
& \text{subject to}
& &  
{\rm SNR}_1 = \eta_1, \quad
% \\
% & & &
{\rm SNR}_2 = \eta_2
% , \quad
% \\
% & & &
% {\bf F}_1 {\bf g}_2 = {\bf 0}.
\label{opt:con}
\end{align}

We assume that User 2 feeds back only the \textit{recent} received signal (i.e., passive feedback) \textit{with  scaling}. In other words,
\begin{equation}
{\bf F}_2 = \begin{bmatrix}
0 & 0 & 0 & ... & 0\\
f_{2,2} & 0 & 0 & ... & 0 \\
0 & f_{2,3} & 0 & ... & 0  \\
\vdots & \vdots & \ddots & & 0 \\
0 & 0 & ... & f_{2,N} & 0
\end{bmatrix} \in \mathbb{C}^{N \times N}.
\end{equation} 

\begin{lemma}
For the optimization problem in \eqref{opt:obj}-\eqref{opt:con}, the optimal solution for $f_{2,N}$ is zero.
\end{lemma}
%
\begin{proof}
We let $\tilde {\bf F}_2$ be equal to ${\bf F}_2$ except that the last entry of $\tilde {\bf F}_2$ is zero, i.e.,  $\tilde f_{2,N}=0$. We then have 
\begin{equation}
    {\rm SNR}_2 = {\bf g}_2^T ({\bf F}_2 {\bf F}_2^T \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} {\bf g}_2 \le {\bf g}_2^T (\tilde {\bf F}_2 \tilde {\bf F}_2^T \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} {\bf g}_2
\end{equation}
For any feasible values of ${\bf g}_2$ and ${\bf F}_2$,
% ${\bf g}_1$, ${\bf F}_1$, ${\bf g}_2$, and ${\bf F}_2$,
% we have the inequalities given by
% \begin{equation}
%     {\rm SNR}_2 = {\bf g}_2^T ({\bf F}_2 {\bf F}_2^T \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} {\bf g}_2 
%     \le {\bf g}_2^T (\tilde {\bf F}_2 \tilde {\bf F}_2^T \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} {\bf g}_2
% \end{equation}
we can always choose $\tilde {\bf g}_2 = (1-\epsilon){\bf g}_2$ with $\epsilon \in [0,1]$ to satisfy  $\tilde {\bf g}_2^T (\tilde {\bf F}_2 \tilde {\bf F}_2^T \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} \tilde {\bf g}_2 = \eta_2$. 
For any feasible values of ${\bf g}_1$, ${\bf F}_1$, ${\bf g}_2$, and ${\bf F}_2$,
we  have a lower bound of $\mathbb{E}\big[\|{\bf x}_2 \|^2\big]$ with $\tilde {\bf g}_2$ and $\tilde {\bf F}_2$, i.e.,
\begin{align}
    \mathbb{E}\big[\|{\bf x}_2 \|^2\big] & = \| ({\bf I} + {\bf F}_2 {\bf F}_1 ) {\bf g}_2\|^2 + \|{\bf F}_2{\bf g}_1\|^2
    + 
    \| {\bf F}_2( {\bf I} + {\bf F}_1{\bf F}_2 ) \|_F^2 \sigma_1^2
    + \| {\bf F}_2{\bf F}_1 \|_F^2 \sigma_2^2  
    \\
    & 
    \ge \| ({\bf I} + \tilde {\bf F}_2 {\bf F}_1 ) \tilde {\bf g}_2\|^2 + \|\tilde {\bf F}_2{\bf g}_1\|^2
    + 
    \| \tilde {\bf F}_2( {\bf I} + {\bf F}_1 \tilde {\bf F}_2 ) \|_F^2 \sigma_1^2
    + \| \tilde {\bf F}_2{\bf F}_1 \|_F^2 \sigma_2^2  
\end{align}
Note that $\mathbb{E}\big[\|{\bf x}_1 \|^2\big]$ and ${\rm SNR}_1$ are not dependent on $f_{2,N}$.
Therefore, 
we can always obtain a smaller (or an equal) objective value in \eqref{opt:obj}
when $f_{2,N}=0$,
% , we can have a smaller objective function value 
while satisfying the SNR constraints.
% Suppose that ${\bf g}_2$ satisfies the SNR constraint, ${\bf g}_2^T ({\bf F}_2 {\bf F}_2^T \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} {\bf g}_2  = \eta_2$.
% For any solutions of ${\bf g}_1$, ${\bf F}_1$, ${\bf g}_2$, and ${\bf F}_2$, we can at least find  the
% smaller value of the objective function by using $a {\bf g}_2$ instead of ${\bf g}_2$ where $a \in [0,1]$.
\end{proof}
The result of the above lemma agrees with the fact that the feedback information transmitted by User 2 at the last channel use is not utilized for the feedback scheme by User 1, and thus is useless.


\begin{lemma}
For the optimization problem in \eqref{opt:obj}-\eqref{opt:con}, 
the optimal solution for ${\bf g}_2$ is ${\bf g}_2^\star = [0, 0, ..., \sqrt{\eta_2}\sigma_2]^T$.
\end{lemma}
%
\begin{proof}
% We have the term $\|{\bf F}_1 {\bf g}_2 \|^2$ in  $\mathbb{E}[\|{\bf x}_1\|^2]$.
% For any values of ${\bf g}_1$, ${\bf F}_1$, ${\bf g}_2$, and ${\bf F}_2$,
Let ${\bf g}_2^\star = [0, 0, ..., \sqrt{\eta_2}\sigma_2]^T$. 
First, ${\bf g}_2^\star$ has the minimum norm among 
any ${\bf g}_2$, i.e., $\| {\bf g}_2^\star  \| \le \| {\bf g}_2  \|$, that satisfies the SNR constraint, ${\bf g}_2^T ({\bf F}_2 {\bf F}_2^T \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} {\bf g}_2 = \eta_2$.
This is due to $f_{2,N}=0$ from Lemma 1. 
% That is, 
% we have $\| {\bf g}_2^\star  \| \le \| {\bf g}_2  \|$ for any ${\bf g}_2$. 
% that satisfies the SNR constraint, i.e., ${\bf g}_2^T ({\bf F}_2 {\bf F}_2^T \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} {\bf g}_2 = \eta_2$,
% First, this value has the minimum norm
% satisfies the SNR constraint, ${\bf g}_2^T ({\bf F}_2 {\bf F}_2^T \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} {\bf g}_2 = \eta_1$, with minimum norm, 
% In other words, we have $\| {\bf g}_2^\star  \| \le \| {\bf g}_2  \|$ for any ${\bf g}_2$ that satisfies the SNR constraint. 
Second, we have ${\bf F}_1 {\bf g}_2^\star = {\bf 0}$ since all the entries in the last column of ${\bf F}_1$ are zero.
% ${{\bf g}_2^\star}T ({\bf F}_2 {\bf F}_2^T \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} {\bf g}_2^\star = \eta_1$, while 
% We have the inequalities given by
% \begin{equation}
%     {\rm SNR}_2 = {\bf g}_2^T ({\bf F}_2 {\bf F}_2^T \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} {\bf g}_2 
%     \le {\bf g}_2^T ({\bf F}_2 {\bf F}_2^T \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} {\bf g}_2
% \end{equation}
With these two properties, for any feasible values of ${\bf F}_1$, ${\bf g}_2$, and ${\bf F}_2$, we have
\begin{equation}
    \|{\bf F}_1 {\bf g}_2 \|^2 \ge \|{\bf F}_1 {\bf g}_2^\star \|^2 = 0
\end{equation}
in $\mathbb{E}[\|{\bf x}_1\|^2]$ and
\begin{align}
    \| ({\bf I} + {\bf F}_2 {\bf F}_1 ) {\bf g}_2\|^2
    & =  \| {\bf g}_2 \|^2 + 2 {\bf g}_2^T {\bf F}_2 {\bf F}_1 {\bf g}_2 + {\bf g}_2^T {\bf F}_1^T {\bf F}_2^T {\bf F}_2 {\bf F}_1  {\bf g}_2
    \\
    & 
    % \ge  \| ({\bf I} + {\bf F}_2 {\bf F}_1 ) {\bf g}_2^\star\|^2 
    \ge \| {\bf g}_2^\star\|^2 = \| ({\bf I} + {\bf F}_2 {\bf F}_1 ) {\bf g}_2^\star\|^2 
\end{align}
in $\mathbb{E}[\|{\bf x}_2\|^2]$. Note that ${\rm SNR}_1$ is not dependent on ${\bf g}_{2}$. 
We conclude that  ${\bf g}_2^\star$ yields the smallest value of the objective function in \eqref{opt:obj} while satisfying the SNR constraints in \eqref{opt:con}. Therefore, ${\bf g}_2^\star$ is the optimal solution for the optimization problem in \eqref{opt:obj}-\eqref{opt:con}.
% The optimal solutions for ${\bf g}_2$ 
% should satisfy ${\bf g}_2^H ({\bf F}_2 {\bf F}_2^H \sigma_1^2 + \sigma_2^2{\bf I} )^{-1} {\bf g}_2 = \eta_2$ and
% ${\bf F}_1 {\bf g}_2 = {\bf 0}$.
% For any general form of ${\bf F}_1$, which is strictly lower triangular, the optimal solution for ${\bf g}_2$ can be found as the vector in which
% only the last entry is non-zero and the rest of entries are zero, i.e., ${\bf g}_2[N] = \sqrt{\eta_2}\sigma_2$ and ${\bf g}_2[k]=0$ for $k=1,...,N-1$.
\end{proof}
The result of the lemma implies that User 2 pours its transmission power into the last channel use 
enough to satisfy the SNR constraint.
\rev{However, the simulations in Sec.~V  show that User 2 can split its power over the empty channel uses  to mitigate the instantaneous power concentration while maintaining the same objective function value. This implies that we can have multiple optimal solutions for ${\bf g}_2$. We will discuss it in detail in Sec.~V.}


% Let us define ${\bf q}_i = {\bf Q}_i^{-1/2} {\bf g}_i$ for $i=1, 2$, where ${\bf Q}_i = ({\bf Q}_i^{1/2})^2$. Then, we have
% \begin{equation}
%     {\rm SNR}_i = \| {\bf q}_i \|^2, \quad \| {\bf g}_i \|^2 = {\bf q}^H_i {\bf Q}_i {\bf q}_i 
% \end{equation}
% Using
% $\| {\bf g}_i \|^2 = {\bf q}^H_i {\bf Q}_i {\bf q}_i $,
Let us define ${\bf q}_1 = {\bf Q}_1^{-1/2} {\bf g}_1$ where ${\bf Q}_1 = ({\bf Q}_1^{1/2})^2$. Then, we have
\begin{equation}
    {\rm SNR}_1 = \| {\bf q}_1 \|^2.
    % , \quad \| {\bf g}_1 \|^2 = {\bf q}^H_1 {\bf Q}_1 {\bf q}_1 
\end{equation}
Using
$\| {\bf g}_1 \|^2 = {\bf q}^H_1 {\bf Q}_1 {\bf q}_1$,
we rewrite the power expressions as
\begin{align}
    \mathbb{E}[\|{\bf x}_1\|^2] 
    &= 
    {\bf q}^H_1 {\bf Q}_1 {\bf q}_1 +
     \|{\bf F}_1 {\bf F}_2 \|_F^2 \sigma_1^2
    + \| {\bf F}_1 \|_F^2 \sigma_2^2
    \\
    &= 
    \|{\bf q}^H_1 ({\bf I} + {\bf F}_1{\bf F}_2) \|^2 \sigma_1^2
    + 
    \| {\bf q}^H_1 {\bf F}_1 \|^2 \sigma_2^2
    + \|{\bf F}_1 {\bf F}_2 \|_F^2 \sigma_1^2
    + \| {\bf F}_1 \|_F^2 \sigma_2^2
    \\
    %%%%%%%%%
    \mathbb{E}[\|{\bf x}_2\|^2] 
    & =  
    % {\bf q}^H_2 {\bf Q}_2 {\bf q}_2 
    \| {\bf g}_2 \|^2
    + \|{\bf F}_2 {\bf Q}_1^{1/2} {\bf q}_1\|^2
    + 
    \| {\bf F}_2({\bf I} + {\bf F}_1{\bf F}_2 ) \|_F^2 \sigma_1^2
    + \| {\bf F}_2 {\bf F}_1
    \|_F^2 \sigma_2^2.
\end{align}

Then, we reduce the optimization into
\begin{align}
    & 
    \underset{{\bf q}_1, {\bf F}_1, {\bf F}_2}
    {\text{minimize}} & & 
 \alpha \mathbb{E}\big[\|{\bf x}_1 \|^2\big] + (1-\alpha) \mathbb{E}\big[\|{\bf x}_2 \|^2\big]
\\
& \text{subject to}
& &  
\| {\bf q}_1\|^2 = \eta_1,  \quad
% \\
% & & &
% \| {\bf q}_2\|^2 \ge \eta_2, \quad
% {\bf F}_1 {\bf Q}_2^{1/2}  {\bf q}_2 = {\bf 0}. 
\end{align}




\section{Solution Method}
% \rev{Revise from here}

We focus on the real case. We propose an iterative method where we solve for ${\bf q}_1$ and ${\bf F}_1$ with ${\bf F}_2$ fixed, and solve for ${\bf F}_2$ with ${\bf q}_1$ and ${\bf F}_1$ fixed.
% \subsection{Solving for ${\bf S}$ and ${\bf q}_1$}

\subsection{Solving for ${\bf q}_1$ and ${\bf F}_1$}

We assume that ${\bf F}_2$ is fixed.
We first focus on solving the unconstrained optimization with respect to  ${\bf F}_1$. Note that ${\bf F}_1$ is a strictly lower triangular matrix given by
\begin{equation}
{\bf F}_1 = \begin{bmatrix}
0 & 0 & 0 & ... & 0\\
f_{1,2,1} & 0 & 0 & ... & 0 \\
f_{1,3,1} & f_{1,3,2} & 0 & ... & 0  \\
\vdots & \vdots & \ddots & & 0 \\
f_{1,N,1} & f_{1,N,2} & ... & f_{1,N,N-1} & 0
\end{bmatrix} = \begin{bmatrix}
0 & 0 & 0 & ... & 0\\
{\bf f}_{1,1} & 0 & 0 & ... & 0 \\
 & {\bf f}_{1,2} & 0 & ... & 0  \\
 &  & \ddots & 0 & 0 \\
 &  & ... & {\bf f}_{1,N-1} & 0
\end{bmatrix}
\in \mathbb{R}^{N \times N},
\end{equation}
where ${\bf f}_{1,i} = [f_{1,i+1,i}, f_{1,i+2,i}, ..., f_{1,N,i}]^T \in \mathbb{R}^{(N-i) \times 1}$, $i=1,...,N-1$.
Note that ${\bf q}_{1} = [q_{1,1}, q_{1,2}, ..., q_{1,N}]^T$.
With this, we define
\begin{equation}
    {\bf h}_{i} = [q_{1,i+1}, q_{1,i+2}, ..., q_{1,N}]^T \in \mathbb{R}^{(N-i) \times 1}, \quad i=0,...,N-1.
\end{equation}
% For notational simplicity, we define ${\bf f}_{1,N} = {\bf f}_{1,N+1} = {\bf h}_{N} = {\bf h}_{N+1} = 0$.

% With these, we express the power of User 1 as
% \begin{align}
%     \mathbb{E}[\|{\bf x}_1\|^2] 
%     &= 
%     \|{\bf q}^T_1 ({\bf S}{\bf F}_2 + {\bf I}) \|^2 \sigma_1^2
%     + 
%     \| {\bf q}^T_1 {\bf S} \|^2 \sigma_2^2
%     + \|{\bf S} {\bf F}_2 \|_F^2 \sigma_1^2
%     + \| {\bf S} \|_F^2 \sigma_2^2
%     \\
%     & = \sigma_1^2 \sum_{i=1}^N \vert q_{1,i} + {\bf h}_{i+1}^T {\bf s}_{i+1} \vert^2 
%     + \sigma_2^2 \sum_{i=1}^N \vert {\bf h}_{i}^T {\bf s}_{i} \vert^2
%     + \sigma_1^2 \sum_{i=2}^N {\bf s}_{i}^T {\bf s}_{i}
%     + \sigma_2^2 \sum_{i=1}^N {\bf s}_{i}^T {\bf s}_{i}
% \end{align}


% \rev{${\bf F}_2$ Approximation should be modified!!}
% We note that 
% % We express the power of User 2 as
% \begin{align}
%     \mathbb{E}[\|{\bf x}_2\|^2] 
%     & =  \| {\bf g}_2 \|^2 + \|{\bf F}_2 {\bf Q}_1^{1/2} {\bf q}_1\|^2
%     + 
%     \| {\bf F}_2({\bf I} + {\bf F}_1{\bf F}_2  ) \|_F^2 \sigma_1^2
%     + \| {\bf F}_2 {\bf F}_1
%     \|_F^2 \sigma_2^2
%     \\
%     & \le \| {\bf g}_2 \|^2 
%     % + {\bf q}_1^T {\bf Q}_1 {\bf q}_1
%     + 
%     Tr({\bf F}_2{\bf F}_2^T) \sigma_1^2 + 
%     \|{\bf F}_1 {\bf F}_2 \|_F^2 \sigma_1^2
%     + \|  {\bf F}_1
%     \|_F^2 \sigma_2^2
%     \\
%     & =  \eta_2 \sigma_2^2 
%     + \| {\bf q}_2^T {\bf F}_2 \|^2 \sigma_1^2   
%     + (N-1) \sigma_1^2
%     + \mathbb{E}[\|{\bf x}_1\|^2] 
% \end{align}
% We then have the upper bound for the original objective function given by
% \begin{equation}
%     \alpha_1 \mathbb{E}\big[\|{\bf x}_1 \|^2\big] + \alpha_2 \mathbb{E}\big[\|{\bf x}_2 \|^2\big] 
%     \le  \alpha_2 (\eta_2 \sigma_2^2 
%     + \| {\bf q}_2^T {\bf F}_2 \|^2 \sigma_1^2 + (N-1) \sigma_1^2) + \mathbb{E}\big[\|{\bf x}_1 \|^2\big]
% \end{equation}
% We instead minimize the upper bound. Then, our optimization problem is


\rev{Need reason or approximation formula.}
We aim to maximize $\mathbb{E}[\|{\bf x}_1\|^2] $, which is expressed as
% by designing  ${\bf q}_1$ and ${\bf F}_1$.
% We express $\mathbb{E}[\|{\bf x}_1\|^2] $ as
\begin{align}
    \mathbb{E}[\|{\bf x}_1\|^2] 
    & = \sigma_1^2 \sum_{i=1}^{N-2} \big\vert q_{1,i} + f_{2,i+1}{\bf h}_{i+1}^T {\bf f}_{1,i+1} \big\vert^2 + \sigma_1^2(q_{1,N-1}^2 + q_{1,N}^2) 
    \\
    & \hspace{.5cm}
    + \sigma_2^2 \sum_{i=1}^{N-1} \vert {\bf h}_{i}^T {\bf f}_{1,i} \vert^2
    + \sigma_1^2 \sum_{i=2}^{N-1} \vert f_{2,i} \vert^2 {\bf f}_{1,i}^T {\bf f}_{1,i}
    + \sigma_2^2 \sum_{i=1}^{N-1} {\bf f}_{1,i}^T {\bf f}_{1,i}
\end{align}

The objective function can be rewritten as
\begin{align}
     \mathbb{E}\big[\|{\bf x}_1 \|^2\big] & = \vert {\bf h}_1^T {\bf f}_{1,1} \vert^2 \sigma_2^2 
     +   {\bf f}_{1,1}^T {\bf f}_{1,1} \sigma_2^2
    \\
    & \hspace{1cm} 
    + \sum_{i=2}^{N-1} \bigg( \big\vert q_{1,i-1} + f_{2,i} {\bf h}_{i}^T {\bf f}_{1,i} \big\vert^2 \sigma_1^2 
    + \vert {\bf h}_{i}^T {\bf f}_{1,i} \vert^2 \sigma_2^2 
    +{\bf f}_{1,i}^T {\bf f}_{1,i}  (\vert f_{2,i} \vert^2 \sigma_1^2 + \sigma_2^2)
    \bigg)
    \nonumber
    \\
    & \hspace{1cm} + \big( \vert q_{1,N-1} \vert^2 + \vert q_{1,N} \vert^2  \big) \sigma_1^2
\end{align}
The objective function can be
decomposed into $N-1$ independent problems with respect to each ${\bf f}_{1,i}$, $i=1,...,N-1$. 
Note that each independent problem is convex in ${\bf f}_{1,i}$. 
Then,
we can find ${\bf f}_{1,i}$ optimally by setting the derivative to zero. Obviously, we have ${\bf f}_{1,1} = {\bf 0}$. For $i=2,...,N-1$,
\begin{align}
    \frac{\partial \mathbb{E}[\|{\bf x}_1\|^2]}{\partial {\bf f}_{1,i}} = (q_{1,i-1} + f_{2,i}{\bf h}_{i}^T {\bf f}_{1,i})^T {\bf h}_{i}^T f_{2,i}\sigma_1^2
    + ({\bf h}_{i}^T {\bf f}_{1,i})^T {\bf h}_{i}^T \sigma_2^2
    +  (  \vert f_{2,i} \vert^2 \sigma_1^2 + \sigma_2^2) {\bf f}_{1,i}^T = {\bf 0}^T
\end{align}
From the above equation, we have
\begin{align}
    (\vert f_{2,i} \vert^2 \sigma_1^2 + \sigma_2^2)({\bf h}_{i} {\bf h}_{i}^T + {\bf I}){\bf f}_{1,i} = - q_{1,i-1} f_{2,i} \sigma_1^2 {\bf h}_{i}
\end{align}
Thus, we have
\begin{align}
    {\bf f}_{1,i} &= - \frac{q_{1,i-1} f_{2,i} \sigma_1^2}{\vert f_{2,i} \vert^2\sigma_1^2 + \sigma_2^2}
    \big( {\bf h}_{i} {\bf h}_{i}^T + {\bf I} \big)^{-1} {\bf h}_{i}
    \\
    &= - \frac{q_{1,i-1} f_{2,i} \sigma_1^2}{\vert f_{2,i} \vert^2 \sigma_1^2 + \sigma_2^2}
    \bigg({\bf I} - \frac{{\bf h}_{i}{\bf h}_{i}^T}
    {1+ \| {\bf h}_{i}\|^2 } \bigg) {\bf h}_{i}
    \\
    &= - \frac{ f_{2,i}\sigma_1^2}{\vert f_{2,i} \vert^2 \sigma_1^2 + \sigma_2^2}
    \frac{q_{1,i-1}}
    {1+ \| {\bf h}_{i}\|^2 }  {\bf h}_{i}
\end{align}
where we used the Sherman–Morrison formula to obtain the second equality.

Putting the optimal values of $\{{\bf f}_{1,i}\}_{i=1}^{N-1}$ in  $\mathbb{E}[\|{\bf x}_1\|^2]$,    
we get
\begin{align}
    \mathbb{E}[\|{\bf x}_1\|^2] 
    &= 
    \sum_{i=2}^{N-1} \bigg[ 
    \bigg( q_{1,i-1} 
     - \frac{ \vert f_{2,i} \vert^2 \sigma_1^2}{\vert f_{2,i} \vert^2\sigma_1^2 + \sigma_2^2}
    \frac{q_{1,i-1} \|{\bf h}_{i}\|^2}
    {1+ \| {\bf h}_{i}\|^2 }  
    \bigg)^2 \sigma_1^2 
    %
    + \bigg( \frac{ f_{2,i}\sigma_1^2}{\vert f_{2,i} \vert^2\sigma_1^2 + \sigma_2^2}
    \frac{q_{1,i-1} \|{\bf h}_{i}\|^2}
    {1+ \| {\bf h}_{i}\|^2 }  \bigg)^2 \sigma_2^2 
    \nonumber
    \\
    & \hspace{1cm}
     + \bigg( \frac{ f_{2,i}\sigma_1^2}{\vert f_{2,i} \vert^2 \sigma_1^2 + \sigma_2^2}
    \frac{q_{1,i-1} }
    {1+ \| {\bf h}_{i}\|^2 }  \bigg)^2 \|{\bf h}_{i}\|^2 (\vert f_{2,i} \vert^2\sigma_1^2 + \sigma_2^2) \bigg]  
    + \big( \vert q_{1,N-1} \vert^2 + \vert q_{1,N} \vert^2  \big) \sigma_1^2
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    \\
    & 
    = \sum_{i=2}^{N-1}  \frac{\sigma_1^2 q_{1,i-1}^2 \big( \vert f_{2,i} \vert^2\sigma_1^2 + \sigma_2^2(1+ \|{\bf h}_{i}\|^2) \big)}
    {(\vert f_{2,i} \vert^2 \sigma_1^2 + \sigma_2^2)(1+ \|{\bf h}_{i}\|^2)} + \big( \vert q_{1,N-1} \vert^2 + \vert q_{1,N} \vert^2  \big) \sigma_1^2
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    % \\
    % & 
    % = \sum_{i=1}^{N}  \frac{\sigma_1^2 q_{1,i}^2 \big( \vert f_{2,i+1} \vert^2\sigma_1^2 + \sigma_2^2(1+ \|{\bf h}_{i+1}\|^2) \big)}
    % {(\vert f_{2,i+1} \vert^2\sigma_1^2 + \sigma_2^2)(1+ \|{\bf h}_{i+1}\|^2)}
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    \\
    % = \sum_{i=2}^{N-1}  \frac{\sigma_1^2 q_{1,i-1}^2 \big( \vert f_{2,i} \vert^2\sigma_1^2 + \sigma_2^2(1+ \|{\bf h}_{i}\|^2) \big)}
    % {(\vert f_{2,i} \vert^2 \sigma_1^2 + \sigma_2^2)(1+ \|{\bf h}_{i}\|^2)} + \big( \vert q_{1,N-1} \vert^2 + \vert q_{1,N} \vert^2  \big) \sigma_1^2
\end{align}
We reduce our optimization problem into
\begin{align}
    & \underset{ {\bf q}_1 }{\text{minimize}} & & 
    % \sum_{i=1}^{N}  \frac{\sigma_1^2 q_{1,i}^2 \big( \vert f_{2,i+1} \vert^2\sigma_1^2 + \sigma_2^2(1+ \|{\bf h}_{i+1}\|^2) \big)}
    % {(\vert f_{2,i+1} \vert^2\sigma_1^2 + \sigma_2^2)(1+ \|{\bf h}_{i+1}\|^2)}
    \sum_{i=1}^{N-2}  \frac{\sigma_1^2 q_{1,i}^2 \big( \vert f_{2,i+1} \vert^2\sigma_1^2 + \sigma_2^2(1+ \|{\bf h}_{i+1}\|^2) \big)}
    {(\vert f_{2,i+1} \vert^2\sigma_1^2 + \sigma_2^2)(1+ \|{\bf h}_{i+1}\|^2)} + \big( \vert q_{1,N-1} \vert^2 + \vert q_{1,N} \vert^2  \big) \sigma_1^2
\\
& \text{subject to}
& &  
\|{\bf q}_1\|^2  = \eta_1
\end{align}
Recall that ${\bf h}_i = [q_{1,i+1}, q_{1,i+2}, ..., q_{1,N}]^T$ for $i=0,...,N-1$.
% , ${\bf h}_N=0$, and ${\bf h}_{N+1}=0$.

Defining $x_i = q_{1,i}^2$, we rewrite the objective function as
\begin{align}
    & \sum_{i=1}^{N-2}  
    \frac{\vert f_{2,i+1} \vert^2 \sigma_1^4 x_i }{{(\vert f_{2,i+1} \vert^2\sigma_1^2 + \sigma_2^2)(1+ x_{i+2} + ... + x_{N})}} 
    + \sum_{i=1}^{N-2} \frac{\sigma_1^2 \sigma_2^2 x_i}{\vert f_{2,i+1} \vert^2\sigma_1^2 + \sigma_2^2}
    + \sigma_1^2 (x_{N-1} + x_{N})  
\end{align}
The compact form using ${\bf x} = [q_{1,1}^2, ..., q_{1,N}^2]^T \in \mathbb{R}^{N \times 1}$  can be formulated as 
\begin{align}
    \sum_{i=1}^{N-1} \frac{{\bf u}_i^T {\bf x} } { 1+ {\bf m}_i^T {\bf x}}
\end{align}
where ${\bf u}_i, {\bf m}_i \ge {\bf 0}$. Note that ${\bf x} \ge {\bf 0}$. 
This is a multi-objective linear fractional programming \cite{}. We exploit existing solution methods to solve for ${\bf x}$.



\subsection{Solving for ${\bf F}_2$}

We assume that ${\bf q}_1$ and ${\bf F}_1$  are fixed.
The optimization problem is
\begin{align}
    & 
    \underset{{\bf F}_2}
    {\text{minimize}} & & 
 \alpha \mathbb{E}\big[\|{\bf x}_1 \|^2\big] + (1-\alpha) \mathbb{E}\big[\|{\bf x}_2 \|^2\big]
% \\
% & \text{subject to}
% & &  
% \| {\bf q}_1\|^2 = \eta_1,  \quad
% \\
% & & &
% \| {\bf q}_2\|^2 \ge \eta_2, \quad
% {\bf F}_1 {\bf Q}_2^{1/2}  {\bf q}_2 = {\bf 0}. 
\end{align}
Recall that 
\begin{equation}
    \mathbb{E}[\|{\bf x}_2\|^2] 
    =  
    % {\bf q}^H_2 {\bf Q}_2 {\bf q}_2 
    \| {\bf g}_2 \|^2
    + \|{\bf F}_2 {\bf Q}_1^{1/2} {\bf q}_1\|^2
    + 
    \| {\bf F}_2({\bf I} + {\bf F}_1{\bf F}_2 ) \|_F^2 \sigma_1^2
    + \| {\bf F}_2 {\bf F}_1
    \|_F^2 \sigma_2^2.
\end{equation}
We will express each of the term including ${\bf F}_2$ as the sum of entries of ${\bf F}_2$.
\begin{align}
     \|{\bf F}_2 {\bf Q}_1^{1/2} {\bf q}_1\|^2 & = {\bf q}_1^T {\bf Q}_1^{1/2} {\bf F}_2^T {\bf F}_2 {\bf Q}_1^{1/2} {\bf q}_1
     \\
     & = {\bf p}^T {\bf F}_2^T {\bf F}_2 {\bf p}
     \\
     & = \sum_{i=2}^N p_{i-1}^2 f_{2,i}^2
\end{align}
where we assume that ${\bf p} := {\bf Q}_1^{1/2} {\bf q}_1$ is fixed although ${\bf Q}_1^{1/2}$ depends on ${\bf F}_2$.
We also have
\begin{align}
     \|{\bf F}_2({\bf I} + {\bf F}_1{\bf F}_2 ) \|_F^2 \sigma_1^2 & = \sigma_1^2 Tr \bigg( {\bf F}_2({\bf I} + {\bf F}_1{\bf F}_2 ) ({\bf I} + {\bf F}_1{\bf F}_2 )^T {\bf F}_2^T  \bigg)
     \\
     & = \sigma_1^2 Tr \bigg( {\bf F}_2 {\bf F}_2^T  \bigg) 
     + 2 \sigma_1^2 Tr \bigg( {\bf F}_2 {\bf F}_1 {\bf F}_2 {\bf F}_2^T \bigg) 
     + \sigma_1^2 Tr \bigg( {\bf F}_2 {\bf F}_1 {\bf F}_2 {\bf F}_2^T {\bf F}_1^T {\bf F}_2^T \bigg)
     \\
     & = \sigma_1^2 \sum_{i=2}^N f_{2,i}^2 + \sigma_1^2 \sum_{i=2}^{N-2} \sum_{j=i+1}^{N-1} f_{1,j,i}^2 f_{2,i}^2 f_{2,j+1}^2
\end{align}
Lastly,
\begin{align}
    \| {\bf F}_2 {\bf F}_1 \|_F^2 \sigma_2^2 
    & = \sigma_2^2 Tr \bigg( {\bf F}_2^T {\bf F}_1^T {\bf F}_1 {\bf F}_2 \bigg)
    \\
    & = \sigma_2^2 \sum_{i=2}^{N-1} \| {\bf f}_{1,i} \|^2 f_{2,i}^2
\end{align}

We will minimize $\alpha \mathbb{E}\big[\|{\bf x}_1 \|^2\big] + (1-\alpha) \mathbb{E}\big[\|{\bf x}_2 \|^2\big]$ for each $f_{2,i}$, $i=2,...,N$ by setting the derivative w.r.t. $f_{2,i}$ equal to zero. 
We have 
\begin{align}
    \frac{\partial \mathbb{E}\big[\|{\bf x}_1 \|^2\big]}{f_{2,i}} 
    % & = 2\sigma_1^2 (q_{1,i-1} + f_{2,i} {\bf h}_i^T {\bf f}_{1,i})  {\bf h}_i^T {\bf f}_{1,i}
    % + 2 \sigma_1^2  {\bf f}_{1,i}^T {\bf f}_{1,i} f_{2,i}
    % \\
    & = 2\sigma_1^2 q_{1,i-1} {\bf h}_i^T {\bf f}_{1,i} + 
    2 \sigma_1^2 \big( \vert {\bf h}_i^T {\bf f}_{1,i} \vert^2    + \| {\bf f}_{1,i} \|^2  \big) f_{2,i}
\end{align}
for $i=2,...,N-1$, and
\begin{align}
    \frac{\partial \mathbb{E}\big[\|{\bf x}_2 \|^2\big]}{f_{2,i}} 
    & = 2 p_{i-1}^2 f_{2,i} + 2 \sigma_1^2 f_{2,i} + 2 \sigma_1^2 f_{2,i} \bigg( \sum_{j=i+1}^{N-1} f_{1,j,i}^2 f_{2,j+1}^2 + \sum_{k=2}^{i-2} f_{1,i-1,k} f_{2,k}^2
    \bigg)
    + 2 \sigma_2^2 \| {\bf f}_{1,i} \|^2 f_{2,i}
\end{align}
Then, we have
\begin{align}
    \alpha \frac{\partial \mathbb{E}\big[\|{\bf x}_1 \|^2\big]}{f_{2,i}}  + (1-\alpha) \frac{\partial \mathbb{E}\big[\|{\bf x}_2 \|^2\big]}{f_{2,i}}  & = 
     2 \alpha \sigma_1^2 q_{1,i-1} {\bf h}_i^T {\bf f}_{1,i}  + c_i f_{2,i} 
\end{align}
where
\begin{align}
    c_i & = 2 \alpha \sigma_1^2 \big( \vert {\bf h}_i^T {\bf f}_{1,i} \vert^2    + \| {\bf f}_{1,i} \|^2  \big) +   2 (1-\alpha) p_{i-1}^2 + 2 (1-\alpha) \sigma_1^2  
    \\
    & \hspace{.5cm} + 2 (1-\alpha) \sigma_1^2  \bigg( \sum_{j=i+1}^{N-1} f_{1,j,i}^2 f_{2,j+1}^2 + \sum_{k=2}^{i-2} f_{1,i-1,k} f_{2,k}^2
    \bigg)
    + 2 \sigma_2^2 (1-\alpha) \| {\bf f}_{1,i} \|^2 
\end{align}
Then, we obtain
\begin{equation}
    f_{2,i} = -\frac{2 \alpha \sigma_1^2 q_{1,i-1} {\bf h}_i^T {\bf f}_{1,i}}{c_i}, \quad i=2,...,N-1
\end{equation}

% \rev{Revise the below: Generalize the below including $f_{2,i}$.}
% \rev{(If $\vert f_{2,i} \vert^2 =1$ for all $i$, then the above optimization can be reduced as below...)}
% We reduce our optimization problem into
% % \rev{(Try linear programming as setting $\alpha_i = \vert v_i \vert^2$)}
% \begin{align}
%     & \underset{ {\bf q}_1 }{\text{minimize}} & & 
%     \sum_{i=1}^N \frac{ q_{1,i}^2}{1+ \|{\bf h}_{i+1} \|^2}
% \\
% & \text{subject to}
% & &  
% \|{\bf q}_1\|^2  = \eta_1
% \end{align}
% Recall that ${\bf h}_i = [q_{1,i+1}, q_{1,i+2}, ..., q_{1,N}]^T$ for $i=0,...,N-1$, ${\bf h}_N=0$, and ${\bf h}_{N+1}=0$.

% From simulations, we observe that when $N$ is odd, the solution of the above optimization problem has the form with $q_{1,i} \approx 0$ for $i = 2, 4, ..., N-1$. Considering this, we will solve the problem by letting $q_{1,i} = 0$ for $i = 2, 4, ..., N-1$. First, we introduce a new variable
% \begin{equation}
%     \delta_i = 1+ \frac{ q_{1,i}^2}{1+ \|{\bf h}_{i+1} \|^2}, \quad i=1, 2, ..., N.
% \end{equation}
% Since $v_{i}=0$ for an even number $i$, we have
% \begin{equation}
%     \delta_i =
%         \begin{cases}
%     1, & \text{if } i = 2, 4, ..., N-1\\
%     \frac{1+ \|{\bf h}_{i-1} \|^2}{1+ \|{\bf h}_{i+1} \|^2},  & \text{if } i = 1, 3, ..., N
% \end{cases}
% \end{equation}
% We can easily deduce that
% \begin{equation}
%     \prod_{i=1}^N \delta_i = 1+ \|{\bf h}_{0} \|^2 = 1 + \eta_1.
% \end{equation}
% Then, we can reduce the problem w.r.t. ${\bf q}_1$ to that w.r.t. $\{\delta_i\}_{i=1}^N$, given by
% \begin{align}
%     & \underset{ \{\delta_i\}_{i=1}^N }{\text{minimize}} & & 
%     \sum_{i=1}^N (\delta_i-1)
% \\
% & \text{subject to}
% & &  
% \prod_{i=1}^N \delta_i = 1 + \eta_1,
% % \\
% % & & & \delta_i=1, \quad i = 2, 4, ..., N-1.
% \end{align}
% The solution of the optimization problem is 
% \begin{equation}
%     \delta_i  =
%     \begin{cases}
%     1, & \text{if } i = 2, 4, ..., N-1\\
%     (1+\eta_1)^{\frac{2}{N+1}},  & \text{if } i = 1, 3, ..., N
% \end{cases}
% \end{equation}
% %
% By plugging $\{{\delta_i}\}$ in the original equations, we find the optimal solutions of ${\bf q}_1$ and ${\bf S}$.



\clearpage

\begin{figure}[t]
% \centering
% \begin{subfigure}[h]{0.49\linewidth}
    \centering
    \includegraphics[width=.5\linewidth]{figures/sumpower_alpha.png}
    % \vspace{-3mm}
    \caption{The plot of $\alpha \mathbb{E}\big[\|{\bf x}_1 \|^2\big] + (1-\alpha) \mathbb{E}\big[\|{\bf x}_2 \|^2\big]$ along $\alpha$ in Gaussian Two-way channels.}
    % \vspace{-7mm}
\end{figure}

Parameter setup: 
$\sigma_1^2 = 1, \quad \sigma_2^2 = 0.5, \quad N=7, \quad \eta_1 = \eta_2 = 10$

``No feedback" refers to the case with two independent one-way channels. ($\|{\bf g}_1\|^2 = \eta_1\sigma_1^2, \|{\bf g}_2\|^2 = \eta_2\sigma_2^2, {\bf F}_1 = {\bf F}_2 = {\bf 0}$)

``Feedback" refers to the proposed iterative solution method.

% 1. We set  ${\bf g}_2[1]= \sqrt{\eta_2 \sigma_2^2}$ and ${\bf g}_2[k]=0$ for $k=2,...,N$. The setup is inspired from numerical observations of ${\bf g}_2$.

% % We solve for ${\bf q}_1$ and ${\bf F}_1$ with randomly generated ${\bf q}_2$ with several trials, and select the best solution set. We then 

% 2. We obtain ${\bf g}_1$ and ${\bf F}_1$ with given ${\bf g}_2$ and ${\bf F}_2$ by using the above solution method, where ${\bf F}_2 = \begin{bmatrix}
% 0 & 0 & 0 & ... & 0\\
% 1 & 0 & 0 & ... & 0 \\
% 0 & 1 & 0 & ... & 0  \\
% \vdots & \vdots & \ddots & & 0 \\
% 0 & 0 & ... & 1 & 0
% \end{bmatrix}$.

% % 2. We set  ${\bf g}_2[1]= \sqrt{\eta_2 \sigma_2^2}$ and ${\bf g}_2[k]=0$ for $k=2,...,N$. The setup is inspired from numerical observations of ${\bf g}_2$.

% 3.  We set ${\bf F}_2[i+1,i] =0$ for $i=2,4,6$, inspired from  numerical observations of ${\bf g}_1$ and ${\bf F}_1$.
% We find the best values for ${\bf F}_2[i+1,i]$, $i=1,3,5$, through random searches.


For example, the obtained solution at $\alpha=0.8$ is
\begin{align}
    {\bf g}_1 & = \begin{bmatrix}
    \rev{1.65}&  0& \rev{1.05}& 0 & \rev{0.70} & 0 & \rev{0.55}
    \end{bmatrix}^T, \quad
    {\bf g}_2 = \begin{bmatrix}
    0 & 0 & 0 & 0 & 0 & 0 & \rev{2.24}
    \end{bmatrix}^T,
    \\
    {\bf F}_1 & = \begin{bmatrix}
0 & 0 & 0 & 0 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & \rev{-.49} & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & \rev{-.33} & 0 & \rev{-.41} & 0 & 0 & 0\\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & \rev{-.25} & 0 & \rev{-.32} & 0 & \rev{-.36}& 0
\end{bmatrix}, \quad
    {\bf F}_2 = \begin{bmatrix}
0 & 0 & 0 & 0 & 0 & 0 & 0\\
\rev{1.00} & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0 \\
0 & 0 & \rev{.89} & 0 & 0 & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0\\
0 & 0 & 0 & 0 & \rev{.68} & 0 & 0 \\
0 & 0 & 0 & 0 & 0 & 0 & 0
\end{bmatrix}
\end{align}

% \clearpage
% \textbf{Other Simulation Results}

\begin{figure}[t]
% \centering
% \begin{subfigure}[h]{0.49\linewidth}
    \centering
    \includegraphics[width=.5\linewidth]{figures/power_dist.png}
    % \vspace{-3mm}
    \caption{Power distribution over channel uses when $N=7$}
    % \vspace{-7mm}
\end{figure}

\begin{figure}[t]
% \centering
% \begin{subfigure}[h]{0.49\linewidth}
    \centering
    \includegraphics[width=.5\linewidth]{figures/sumpower_N.png}
    % \vspace{-3mm}
    \caption{The plot of $\alpha \mathbb{E}\big[\|{\bf x}_1 \|^2\big] + (1-\alpha) \mathbb{E}\big[\|{\bf x}_2 \|^2\big]$ along $N$}
    % \vspace{-7mm}
\end{figure}


\begin{figure}[t]
\centering
\begin{subfigure}[h]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/sumpower_np1.png}
    \caption{$\sigma_1^2$}
\end{subfigure}
%%%%%
\begin{subfigure}[h]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/sumpower_np2.png}
    \caption{$\sigma_2^2$}
\end{subfigure}
\caption{The plot of $\alpha \mathbb{E}\big[\|{\bf x}_1 \|^2\big] + (1-\alpha) \mathbb{E}\big[\|{\bf x}_2 \|^2\big]$ along noise powers}
\end{figure}


